An Exam-based Evaluation Approach Beyond Traditional Relevance Judgments

Current IR evaluation is based on relevance judgments, created either manually or automatically, with decisions outsourced to Large Language Models (LLMs). We offer an alternative paradigm, that never relies on relevance judgments in any form. Instead, a text is defined as relevant if it contains information that enables the answering of key questions. We use this idea to design the EXAM Answerability Metric to evaluate information retrieval/generation systems for their ability to provide topically relevant information. We envision the role of a human judge to edit and define an exam question bank that will test for the presence of relevant information in text. We support this step by generating an initial set of exam questions. In the next phase, an LLM-based question answering system will automatically grade system responses by tracking which exam questions are answerable with which system responses. We propose two evaluation measures, the recall-oriented EXAM Cover metric, and the precision-oriented EXAM Qrels metric, the latter which can be implemented with trec_eval. This paradigm not only allows for the expansion of the exam question set post-hoc but also facilitates the ongoing evaluation of future information systems, whether they focus on retrieval, generation, or both.

==> results/exam_post_pipeline-analysis.txt.tex <==

\section{CAR Y3 - TQA / Answer checking }

\begin{verbatim}

## Inter-annotator

# squad2-finetuned model name:  sjrhuschlee/flan-t5-large-squad2



### Use T5 answer corrected files   ###

QA/Squad2:
result_car_qa="/mnt/cherries/datasets/trec-car-data/additional/answerT5corrected_squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz"

# QA
exp="car-tqa-qa-v5"
prompt="QuestionCompleteConcisePromptWithT5VerifiedAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out "leaderboard-${exp}.tsv" --correlation-out "correlation--${exp}.tex" --qrel-query-facets -q "qrel-${exp}.qrels"  > "${exp}-analysis.log"

#min_rating=None nExam:CorrelationStats(spearman_correlation=0.7313103409735259, kendall_correlation=0.5493612827995783)
# min_rating=None  exam:CorrelationStats(spearman_correlation=0.7150261026117674, kendall_correlation=0.5321937427120915)



#Squad2
exp="car-tqa-squad2-v5"
prompt="QuestionCompleteConcisePromptWithT5VerifiedAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model sjrhuschlee/flan-t5-large-squad2 --leaderboard-out leaderboard-${exp}.tsv --correlation-out correlation--${exp}.tex  --qrel-query-facets -q "qrel-${exp}.qrels" > "${exp}-analysis.log"

min_rating=None nExam:CorrelationStats(spearman_correlation=0.8660254037844386, kendall_correlation=0.7553717638494203)
min_rating=None  exam:CorrelationStats(spearman_correlation=0.8630646331732098, kendall_correlation=0.7382042237619334)


# CC:
result_car_cc="/mnt/cherries/datasets/trec-car-data/additional/answerT5corrected_t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"

exp="car-tqa-cc-v5"
prompt="QuestionCompleteConcisePromptWithT5VerifiedAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_cc  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out leaderboard-${exp}.tsv --correlation-out correlation--${exp}.tex  --qrel-query-facets -q "qrel-${exp}.qrels" > "${exp}-analysis.log"

min_rating=None nExam:CorrelationStats(spearman_correlation=0.877868486229354, kendall_correlation=0.7210366836744466)
min_rating=None  exam:CorrelationStats(spearman_correlation=0.877868486229354, kendall_correlation=0.7210366836744466)

## ---



Use nltk answer corrected files

QA/Squad2:  answercorrected-squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz
CC: answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz
--prompt-class QuestionCompleteConcisePromptWithAnswerKey2


--------------

Anwer corrected

QA/Squad2:

result_car_qa="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz"
result_car_qa="answercorrected-squad2-t5-qa-tqa-exam--benchmarkY3test-exam-qrels-runs-with-text.jsonl.gz"

# QA
exp="car-tqa-qa-corrected"
prompt="QuestionCompleteConcisePromptWithAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out "leaderboard-${exp}.tsv" --correlation-out "correlation--${exp}.tex" --qrel-query-facets -q "qrel-${exp}.qrels"  > "${exp}-analysis.log"

mkdir datax
ls *${exp}*
cp *${exp}* datax/


#Squad2
exp="car-tqa-squad2-corrected"
prompt="QuestionCompleteConcisePromptWithAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class $prompt --question-set tqa  --testset cary3   --model sjrhuschlee/flan-t5-large-squad2 --leaderboard-out "leaderboard-${exp}.tsv" --correlation-out "correlation--${exp}.tex" --qrel-query-facets -q "qrel-${exp}.qrels"  > "${exp}-analysis.log"
cp *${exp}* datax/

# CC:
# result_car_cc="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"
result_car_cc="answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"

exp="car-tqa-cc-corrected"
prompt="QuestionCompleteConcisePromptWithAnswerKey2"
python -O -m exam_pp.exam_post_pipeline $result_car_cc  --prompt-class $prompt --question-set tqa  --testset cary3   --model google/flan-t5-large --leaderboard-out leaderboard-${exp}.tsv --correlation-out correlation--${exp}.tex  --qrel-query-facets -q "qrel-${exp}.qrels" > "${exp}-analysis.log"

cp *${exp}* datax/

% -------------

% #### Correlation/Leaderboard #####

% #Squad2

% python -O -m exam_pp.exam_post_pipeline $result_car_qa  --prompt-class QuestionCompleteConcisePromptWithAnswerKey2 --question-set tqa  --testset cary3 --model sjrhuschlee/flan-t5-large-squad2 --leaderboard-out leaderboard-car-tqa-squad2.tsv 


% Exam-Cover leaderboard (answer-corrected)
% CC
% min_rating=None  exam:CorrelationStats(spearman_correlation=0.9370838984539311, kendall_correlation=0.8412094642868543)


% QA 
% min_rating=None  exam:CorrelationStats(spearman_correlation=0.8230942299216203, kendall_correlation=0.6695340634119862)

% Squad2
% min_rating=None  exam:CorrelationStats(spearman_correlation=0.8378980829777646, kendall_correlation=0.6867016034994731)



% ************************
% *  Bug in code, all 0! *
% ************************


\end{verbatim}





\section{CAR Y3 - TQA}
\begin{verbatim}
#result_car="/mnt/cherries/datasets/trec-car-data/additional/t5-rating-naghmehs-tqa-exam-qrel-runs-result.jsonl.gz"
#result_car="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-t5-rating-naghmehs-tqa-exam-qrel-runs-result.jsonl.gz"

runs_car="/mnt/cherries/datasets/trec-car-data/benchmarkY3test-runs-and-more/run/"


#### EXAM-Qrels  #### 
not applicable (because we have faceted run files, but no faceted qrels)


#### Inter-annotator ######
# TQA

# Use Ratings

python -O -m exam_pp.exam_post_pipeline $result_car --correlation-out correlation-car-tqa-self-rating.tex --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set tqa  --testset cary3  --use-ratings 

using min_answers=2: ./result/correlation-car-tqa-self-rating--min-answers-2.tex 


#### Leaderboard Correlation ######
# TQA

# Use Self-ratings
exp="car-tqa-self-rating"
python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set tqa  --testset cary3  --use-ratings   --leaderboard-out leaderboard-${exp}$-4.tsv --min-self-rating 4  --correlation-out correlation-${exp}.tex


min_rating=4 nExam:CorrelationStats(spearman_correlation=0.9252408160090155, kendall_correlation=0.789706844024394)
min_rating=4  exam:CorrelationStats(spearman_correlation=0.9222800453977867, kendall_correlation=0.7725393039369071)

./results/leaderboard-car-tqa-self-rating-4.tsv

Column TQA/Exam in latex table ./result/car-y3-leaderboard-correlation.tex

## CompleteAndConcise

% grading more runs with this command
% stdbuf -oL -eL  python -m exam_pp.exam_grading  -o t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz  $result_car --model-pipeline text2text --model-name google/flan-t5-large --prompt-class QuestionCompleteConcisePromptWithAnswerKey --question-path ./tqa_train_val_test --question-type tqa >examscore.log 2>&1  &



\end{verbatim}


\section{CAR Y3 - Davinci }

\begin{verbatim}
result_davinci_car="/mnt/cherries/datasets/trec-car-data/additional/davinci-cc-self-rated-naghmeh--cc-self-rated-tqa--exam.jsonl.gz"


# self-rating

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set tqa  --testset cary3  --use-ratings   --leaderboard-out leaderboard-davinci-tqa-self-rating-4.tsv --min-self-rating 4 --official-leaderboard empty_leaderboard.json

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings   --leaderboard-out leaderboard-davinci-naghmeh-self-rating-4.tsv --min-self-rating 4 --official-leaderboard empty_leaderboard.json


# cc

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionCompleteConcisePromptWithAnswerKey --question-set tqa  --testset cary3    --leaderboard-out leaderboard-davinci-tqa-cc.tsv --official-leaderboard empty_leaderboard.json


************************
*  Bug in code, all 0! *
************************

python -O -m exam_pp.exam_post_pipeline $result_davinci_car --use-ratings  --prompt-class QuestionCompleteConcisePromptWithAnswerKey --question-set naghmeh  --testset cary3    --leaderboard-out leaderboard-davinci-tqa-cc.tsv --official-leaderboard empty_lea


************************
*  Bug in code, all 0! *
************************


\end{verbatim}

\section{CAR Y3 - GenQuestions}

\begin{verbatim}
% result_car="/mnt/cherries/datasets/trec-car-data/additional/t5-rating-naghmehs-exam-qrel-runs-result.json.gz"
result_car="/mnt/cherries/datasets/trec-car-data/additional/answercorrected-t5-rating-naghmehs-tqa-rating-cc-exam-qrel-runs-result.jsonl.gz"

runs_car="/mnt/cherries/datasets/trec-car-data/benchmarkY3test-runs-and-more/run/"

## EXAM-Qrels, Inter-annotator, Leaderboard 

exp="car-naghmeh-self-rating"
 python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings -q qrel-${exp}.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3 --qrel-query-facets --use-ratings  --run-dir $runs_car  --correlation-out correlation-${exp}.tex --leaderboard-out leaderboard-${exp}-4.tsv --min-self-rating 4 --qrel-leaderboard-out qrel-leaderboard-${exp}.tsv > ${exp}-analysis.log

 
% #### EXAM-Qrels  #### 

% # Naghmeh's question set  (using facets)

%  python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings -q out-complete.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3 --qrel-query-facets --use-ratings  --run-dir $runs_car
 



% #### Inter-annotator ######
% # Naghmeh's questions

% python -O -m exam_pp.exam_post_pipeline $result_car --correlation-out correlation-car-naghmeh-self-rating.tex --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings 

% using min_answers=2:  /results/correlation-car-naghmeh-self-rating--min-answers-2.tex



% #### Leaderboard Correlation ######
% # Naghmeh's questions

% # Use Self-ratings

% python -O -m exam_pp.exam_post_pipeline $result_car --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings   --leaderboard-out leaderboard-car-naghmeh-self-rating-4.tsv --min-self-rating 4


% min_rating=4 nExam:CorrelationStats(spearman_correlation=0.8689861743956674, kendall_correlation=0.6867016034994731)
% min_rating=4  exam:CorrelationStats(spearman_correlation=0.8689861743956674, kendall_correlation=0.6867016034994731)


% ./results/leaderboard-car-naghmeh-self-rating-4.tsv

% Column GenQ/Exam in latex table ./result/car-y3-leaderboard-correlation.tex


\end{verbatim}

\section{CAR Y3 - flan-t5-small}

\begin{verbatim}

#### Leaderboard Correlation ######
# Naghmeh's questions

# Use Self-ratings

result_car_t5small="/mnt/cherries/datasets/trec-car-data/additional/t5small-rating-naghmeh--exam-qrels-runs.jsonl.gz"

python -O -m exam_pp.exam_post_pipeline $result_car_t5small --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set naghmeh  --testset cary3  --use-ratings   --leaderboard-out leaderboard-car-naghmeh-t5small-self-rating-4.tsv --min-self-rating 4

min_rating=4 nExam:CorrelationStats(spearman_correlation=0.31532207009587254, kendall_correlation=0.29184818148727604)
min_rating=4  exam:CorrelationStats(spearman_correlation=0.31532207009587254, kendall_correlation=0.29184818148727604)

\end{verbatim}



\section {DL19}

\begin{verbatim}

result_dl="/home/nf1104/work/dl19_results_examGrading/result_trecDL2019-qrels-runs-with-text__new_subqueries_v2__large_2.jsonl.gz"

% runs_dl="/home/nf1104/work/trec-dl-2019/runs/dl19_runs" --- this path does not exist
runs_dl="/mnt/cherries/home/nf1104/work/trec-dl-2019/runs"
commands

######



% this command is incomplete
% python -O -m exam_pp.exam_post_pipeline $result_dl --use-ratings -q out-complete.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl19  --use-ratings  --run-dir $runs_dl

python -O -m exam_pp.exam_post_pipeline $result_dl --use-ratings -q dl19-exam-3.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl19  --use-ratings  --run-dir $runs_dl --min-trec-eval-level 3 --qrel-leaderboard-out leaderboard-dl19-qrels-genq-self-rating-3.tsv



#####

python -O -m exam_pp.exam_post_pipeline $result_dl --correlation-out correlation-dl19-subqueries-self-rating.tex --use-ratings  --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl19  --use-ratings 

 using min_answers=2: /results/correlation-dl19-self-rating--min-answers-2

#######
#######
#######
files with prompts:


exp="dl19"
result_dl19="/home/nf1104/work/prompt_results/prompt_grades_dl19_correct_answered.jsonl.gz"
runs_dl19="/home/nf1104/work/trec-dl-2019/runs"


cls_values=("FagB" "FagB_few" "Sun" "Sun_few" "HELM" "Thomas")
for cls in "${cls_values[@]}"; do
    # Run the command for each cls value
    python -O -m exam_pp.exam_post_pipeline "$result_dl19" \
        --use-relevance-prompt \
        --trec-eval-qrel-correlation "/home/nf1104/work/qrels/${cls}-${exp}.qrel" \
        --question-set question-bank \
        --testset "$exp" \
        --run-dir "$runs_dl19" \
        --prompt-class "$cls" \
        --correlation-out "./prompted_results/correlation-${cls}-${exp}.tex" \
        --leaderboard-out "./prompted_results/leaderboard-${cls}-${exp}.tsv" \
        --qrel-leaderboard-out "./prompted_results/qrel-leaderboard-${cls}-${exp}.tsv" \
        > "${cls}-analysis.log"
done



#######
exp="dl20"
result_dl20="/home/nf1104/work/prompt_results/prompt_grades_dl20_correct_answered.jsonl.gz"
runs_dl20="/home/nf1104/work/trec-dl-2020/runs"

python -O -m exam_pp.exam_post_pipeline $result_dl20 --use-ratings -q dl20-exam-4.qrels --prompt-class QuestionSelfRatedUnanswerablePromptWithChoices --question-set question-bank  --testset dl20  --use-ratings  --run-dir $runs_dl20 --min-trec-eval-level 4 --qrel-leaderboard-out leaderboard-dl20-qrels-genq-self-rating-4.tsv



cls_values=("FagB" "FagB_few" "Sun" "Sun_few" "HELM" "Thomas")

cls_values=("FagB" "FagB_few" "Sun" "Sun_few" "HELM" "Thomas")
for cls in "${cls_values[@]}"; do
    # Run the command for each cls value
    python -O -m exam_pp.exam_post_pipeline "$result_dl20" \
        --use-relevance-prompt \
        --trec-eval-qrel-correlation "/home/nf1104/work/qrels/${cls}-${exp}.qrel" \
        --question-set question-bank \
        --testset "$exp" \
        --run-dir "$runs_dl20" \
        --prompt-class "$cls" \
        --correlation-out "./prompted_results/correlation-${cls}-${exp}.tex" \
        --leaderboard-out "./prompted_results/leaderboard-${cls}-${exp}.tsv" \
        --qrel-leaderboard-out "./prompted_results/qrel-leaderboard-${cls}-${exp}.tsv" \
        > "${cls}-analysis.log"
done
\end{verbatim}
